Vehicular Applications of Koopman Operator Theory -- A Survey

Koopman operator theory has proven to be a promising approach to nonlinear system identification and global linearization. For nearly a century, there had been no efficient means of calculating the Koopman operator for applied engineering purposes. The introduction of a recent computationally efficient method in the context of fluid dynamics, which is based on the system dynamics decomposition to a set of normal modes in descending order, has overcome this long-lasting computational obstacle. The purely data-driven nature of Koopman operators holds the promise of capturing unknown and complex dynamics for reduced-order model generation and system identification, through which the rich machinery of linear control techniques can be utilized. Given the ongoing development of this research area and the many existing open problems in the fields of smart mobility and vehicle engineering, a survey of techniques and open challenges of applying Koopman operator theory to this vibrant area is warranted. This review focuses on the various solutions of the Koopman operator which have emerged in recent years, particularly those focusing on mobility applications, ranging from characterization and component-level control operations to vehicle performance and fleet management. Moreover, this comprehensive review of over 100 research papers highlights the breadth of ways Koopman operator theory has been applied to various vehicular applications with a detailed categorization of the applied Koopman operator-based algorithm type. Furthermore, this review paper discusses theoretical aspects of Koopman operator theory that have been largely neglected by the smart mobility and vehicle engineering community and yet have large potential for contributing to solving open problems in these areas.

==> table2.tex <==
\definecolor{Gray}{gray}{0.85}
%\definecolor{LightCyan}{rgb}{0.88,1,1}
\setlength{\dashlinedash}{0.3pt}
\setlength\dashlinegap{1.5pt}
%\renewcommand{\arraystretch}{1.05}% More Row Height
\begin{table}[t]
	\caption{Summary of studies organized by the utilized Koopman operator-based algorithm}
	%\centering
	\begin{tabular}{c | c}
		\hline
		\rowcolor{Gray}
		\centering\textbf{Algorithm} & \textbf{Studies$^\ddag$} \\ \hline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
				Projection Methods onto Selected/Derived/Required Basis, including use of Principle Orthogonal Decomposition (POD)
			\vspace{1ex}
		\end{minipage}
		%
		&
		\begin{minipage}{0.1\textwidth}
			\cite{hofmann:2022}\cite{qian:2020}\cite{renganathan:2018}\\
			\cite{otto:2022}  
		\end{minipage}
		%
		\\ \hdashline
		\rowcolor{LightCyan} 
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Dynamic Mode Decomposition (DMD), excluding where DMD is compared against modified methods
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
		\cite{cohen:2021}\cite{schmid:2022}\cite{wu:2021}\\
		\cite{ling:2020}\cite{ling:2018} \cite{boudali:2017}\\
		\cite{hanke:2018}\cite{le:2015}\cite{vasisht:2020} \\
		\cite{journell:2020}\cite{luong:2021}\cite{larusson:2014}\\
		\cite{avila:2021} \cite{manzoor:2022b}  
		\end{minipage}
		\\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
				Extended DMD (EDMD) or slightly modified EDMD, e.g., Naturally Structured DMD (NSDMD)
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{zhu:2022}\cite{berrueta:2020}\cite{schmid:2022}\\
			\cite{cibulka:2019}\cite{vsvec:2021a}\cite{mi:2022}\\
			\cite{vsvec:2021b}\cite{zinage:2022a}\cite{buzhardt:2022}\\
			\cite{lehmberg:2021}\cite{bhandari:2021}\cite{li:2021}\\
			\cite{williams:2016}\cite{calderon:2022}\cite{bruder:2021}\\
			\cite{shi:2021}\cite{chen:2021}\cite{williams:2015}\\
			\cite{moyalan:2022}\cite{broad:2020}\cite{broad:2018}\\
			\cite{pan:2021}
		\end{minipage}
		\\ \hdashline
		\rowcolor{LightCyan} 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			 Weighted Online EDMD (WOEDMD)
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			  \cite{guo:2022}  
		\end{minipage}
		\\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
		DMD with Control (DMDc) 
			\vspace{1ex}
		\end{minipage}
		& 
		%
		\begin{minipage}{0.1\textwidth}
		 \cite{jin:2020}\cite{manzoor:2022b} 
		\end{minipage}
		%
		\\ \hdashline
		%
		\rowcolor{LightCyan}
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Koopman Eigenfunction Extended Dynamic Mode Decomposition (KEEDMD) or modified KEEDMD
			\vspace{1ex} 
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{folkestad:2020a}\cite{folkestad:2020b}  
		\end{minipage}
		\\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Rescaled DMD (rDMD) 
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{cohen:2021}  
		\end{minipage}
		\\ \hdashline
		% 
		\rowcolor{LightCyan} 
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Debiased DMD, Forward/Backward DMD
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			 \cite{schmid:2022}
		\end{minipage}	
		\\ \hline
	\end{tabular}
	\footnotesize \raggedright{$^\ddag$ Detail descriptions are provided in the text.}
	\label{tab2}
\end{table}

==> table3.tex <==
\definecolor{Gray}{gray}{0.85}
%\definecolor{LightCyan}{rgb}{0.88,1,1}
\setlength{\dashlinedash}{0.3pt}
\setlength\dashlinegap{1.5pt}
%\renewcommand{\arraystretch}{1.05}% More Row Height
\begin{table*}[t]
	%\centering
	\caption{Summary of studies organized by the utilized Koopman operator-based algorithm.}
	\begin{tabular}{c | c | c | c}
		\hline
		\rowcolor{Gray}
		\centering\textbf{Algorithm} & \textbf{Studies$^\ddag$} & \centering\textbf{Algorithm} & \textbf{Studies$^\ddag$} \\ \hline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
				Debiased DMD, Forward/Backward DMD 
			\vspace{1ex}
		\end{minipage}
		%
		&
		\begin{minipage}{0.1\textwidth}
			\cite{schmid:2022} 
		\end{minipage}
		%
		& 
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Deep Koopman, Deep Direct Koopman, or other general Artificial Neural Network (ANN) Scheme 
			\vspace{1ex}
		\end{minipage}
		& 
		%
		\begin{minipage}{0.1\textwidth}
			\vspace{0.5ex}
			\cite{xiao:2021_i13}\cite{xiao:2022}\cite{wang:2021}\\
			\cite{han:2020} \cite{wang:2022}\cite{bakker:2020}\\
			\cite{zhan:2022}\cite{maksakov:2020} \cite{jin:2020} 
			\vspace{0.5ex}
		\end{minipage}
		%
		\\ \hdashline
		%
		\rowcolor{LightCyan} 
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Multi-resolution DMD (mrDMD) 
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{schmid:2022}\cite{sullivan:2021} 
		\end{minipage}
	    & 
	     \begin{minipage}{0.33\textwidth}
	    	\vspace{1ex}
	    	Neural Koopman Lyapunov Control [ANN]   
	    	\vspace{1ex}
	    \end{minipage}
	    & 
	    \begin{minipage}{0.1\textwidth}
	    	\cite{zinage:2022b}  
	    \end{minipage}
		\\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			HAVOK, Hankel DMD (partial or full-predictive)  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{schmid:2022}\cite{ali:2021}\cite{haggerty:2020}\\
			\cite{ma:2022}\cite{manzoor:2022a} 
		\end{minipage}
	    & 
	    \begin{minipage}{0.33\textwidth}
	    	\vspace{1ex}
	    	Deterministic/Convolutional Koopman Network (DCKNet, CKNet), Deep Convolutional  Koopman Network (DKN)   
	    	\vspace{1ex}
	    \end{minipage}
	    &
	    \begin{minipage}{0.1\textwidth}
	    	\cite{xiao:2021_i31}\cite{leask:2021}
	    \end{minipage}
	    \\ \hdashline
		\rowcolor{LightCyan} 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Higher-order DMD (HODMD) 
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
		\cite{schmid:2022}\cite{le:2019} 
		\end{minipage}
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Deep Learning with Recurrent Neural Network  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{bieker:2020} 
		\end{minipage}
		
		\\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Physics-based Higher-order EDMD 
			\vspace{1ex}
		\end{minipage}
		& 
		%
		\begin{minipage}{0.1\textwidth}
		\cite{castano:2020}
		\end{minipage}
		%
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Direct Koopman Reinforcement Learning (DKRL) 
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{songy:2021}
		\end{minipage}
		\\ \hdashline
		%
		\rowcolor{LightCyan}
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
		Bilinear EDMD (bEDMD) 
		\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{folkestad:2021}   
		\end{minipage}
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Split Koopman Autoencoder  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{girgis:2021}
		\end{minipage}
		%
		\\ \hdashline
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
				Constant Energy Multiscale DMD (CEM-DMD)
				\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{li:2021}
		\end{minipage}
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Stepwise Akaike Information Criteria (SAIC)  
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{matpan:2021}
		\end{minipage}
		\\ \hdashline
		% 	%	  \\ \hdashline
		\rowcolor{LightCyan} 
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Exact DMD, ANN-based Exact DMD  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{schmid:2022}\cite{li:2021}
		\end{minipage}
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			EDMD with Autodidact Stiffness Learning 
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{goyal:2022}  
		\end{minipage}
		\\ \hdashline
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			LIR-DMD 
			\vspace{1ex}
		\end{minipage}
		%
		&
		\begin{minipage}{0.1\textwidth}
			\cite{li:2021}
		\end{minipage}
	    & 
	    \begin{minipage}{0.33\textwidth}
	    	\vspace{1ex}
	    	Sparse Identification of Nonlinear Dynamics (SINDy) 
	    	\vspace{1ex}
	    \end{minipage}
	    &
	    \begin{minipage}{0.1\textwidth}
	    	\cite{brunton:2016}\cite{matpan:2021} 
	    \end{minipage}
		%
		\\ \hdashline
		\rowcolor{LightCyan} 
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Time Delay DMD (TD-DMD) 
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{pan:2021} 
		\end{minipage}
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Stochastic Koopman Operator (SKO), or Stochastic Adversarial Koopman Operator with Auxillary Neural Network, Gaussian Process-based Koopman Operator, or other Stochastic Methods   
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{balakrishnan:2021}\cite{yingzhao:2020}\\\cite{bujorianu:2021}
			\cite{williams:2015}
		\end{minipage}
	   \\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Kernel DMD (KDMD)  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{pan:2021}
		\end{minipage}
		& 
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Sparcity Promoting DMD (spDMD)   
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{pan:2021}
		\end{minipage}
		\\ \hline
	\end{tabular}
    \newline
	\footnotesize{$^\ddag$ Detail descriptions are provided in the text.}
	 \label{tab3}
\end{table*}


==> table4.tex <==
\definecolor{Gray}{gray}{0.85}
%\definecolor{LightCyan}{rgb}{0.88,1,1}
\setlength\dashlinegap{1.5pt}
%\renewcommand{\arraystretch}{1.05}% More Row Height
\begin{table}[t]
	%\centering
	\caption{Summary of studies organized by the utilized Koopman operator-based algorithm.}
	\begin{tabular}{c | c}
		\hline
		\rowcolor{Gray}
		\centering\textbf{Algorithm} & \textbf{Studies$^\ddag$} \\ \hline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			 Deep Koopman, Deep Direct Koopman, or other general Artificial Neural Network (ANN) Scheme 
			\vspace{1ex}
		\end{minipage}
		& 
		%
		\begin{minipage}{0.1\textwidth}
			\vspace{0.5ex}
			\cite{xiao:2021_i13}\cite{xiao:2022}\cite{wang:2021}\\
			\cite{han:2020} \cite{wang:2022}\cite{bakker:2020}\\
			\cite{zhan:2022}\cite{maksakov:2020} \cite{jin:2020} 
			\vspace{0.5ex}
		\end{minipage}
		%
		\\ \hdashline
		%
		\rowcolor{LightCyan}
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Neural Koopman Lyapunov Control [ANN]   
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			 \cite{zinage:2022b}  
		\end{minipage}
		\\ \hdashline
		%
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Deterministic/Convolutional Koopman Network (DCKNet, CKNet), Deep Convolutional  Koopman Network (DKN)   
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{xiao:2021_i31}\cite{leask:2021}
		\end{minipage}
		\\ \hdashline
		% 	%	  \\ \hdashline
		\rowcolor{LightCyan} 
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Deep Learning with Recurrent Neural Network  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{bieker:2020} 
		\end{minipage}
		
		\\ \hdashline
		
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Direct Koopman Reinforcement Learning (DKRL) 
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{songy:2021}
		\end{minipage}
		\\ \hdashline
		% 	%	  \\ \hdashline
		\rowcolor{LightCyan} 
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Split Koopman Autoencoder  
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{girgis:2021}
		\end{minipage}
		
		\\ \hdashline
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Stepwise Akaike Information Criteria (SAIC)  
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			 \cite{matpan:2021}
		\end{minipage}
		\\ \hdashline
		% 	%	  \\ \hdashline
		\rowcolor{LightCyan} 
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			EDMD with Autodidact Stiffness Learning 
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{goyal:2022}  
		\end{minipage}
		
		\\ \hdashline
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Sparse Identification of Nonlinear Dynamics (SINDy) 
			\vspace{1ex}
		\end{minipage}
		&
		\begin{minipage}{0.1\textwidth}
			\cite{brunton:2016}\cite{matpan:2021} 
		\end{minipage}
		\\ \hdashline
		% 	%	  \\ \hdashline
		\rowcolor{LightCyan} 
		
		\begin{minipage}{0.33\textwidth}
			\vspace{1ex}
			Stochastic Koopman Operator (SKO), or Stochastic Adversarial Koopman Operator with Auxillary Neural Network, Gaussian Process-based Koopman Operator, or other Stochastic Methods   
			\vspace{1ex}
		\end{minipage}
		& 
		\begin{minipage}{0.1\textwidth}
			\cite{balakrishnan:2021}\cite{yingzhao:2020}\\\cite{bujorianu:2021}
			\cite{williams:2015}
		\end{minipage}
		
		\\ \hline
	\end{tabular}
	\footnotesize \raggedright{$^\ddag$ Detail descriptions are provided in the text.}
	 \label{tab4}
\end{table}
